Vid2Curve: Simultaneous Camera Motion Estimation and Thin Structure Reconstruction from an RGB Video

Thin structures, such as wire-frame sculptures, fences, cables, power lines, and tree branches, are common in the real world. It is extremely challenging to acquire their 3D digital models using traditional image-based or depth-based reconstruction methods because thin structures often lack distinct point features and have severe self-occlusion. We propose the first approach that simultaneously estimates camera motion and reconstructs the geometry of complex 3D thin structures in high quality from a color video captured by a handheld camera. Specifically, we present a new curve-based approach to estimate accurate camera poses by establishing correspondences between featureless thin objects in the foreground in consecutive video frames, without requiring visual texture in the background scene to lock on. Enabled by this effective curve-based camera pose estimation strategy, we develop an iterative optimization method with tailored measures on geometry, topology as well as self-occlusion handling for reconstructing 3D thin structures. Extensive validations on a variety of thin structures show that our method achieves accurate camera pose estimation and faithful reconstruction of 3D thin structures with complex shape and topology at a level that has not been attained by other existing reconstruction methods.

==> 4_method_backup.tex <==
\section{Algorithm}
\label{sec:algo}

\subsection{Preprocessing}
\label{sec:preprocess}
%
During preprocessing, we first segment each input image to obtain a binary mask of the pixels showing the thin structure in the foreground. Reliable segmentation of thin structures from a general background is extremely challenging. 
%a difficult and outstanding issue, 
We assume that the 3D thin structure is filmed in front of a simple uniform background so it can be segmented using color keying method or advanced video object segmentation tool such as Rotobrush in Adobe After Effects~\cite{Bai:sigg:2009}. For the shapes of small to medium size, this can be easily achieved by filming in front of a monochromatic wall or cloth. 
%
Let $\inputI=\{\inputIk{k}, k=1 \sim \frameNum\}$ denote the input video as a sequence of RGB frames, and let $\segI=\{\segIk{k}, k=1 \sim \frameNum\}$ denote the corresponding foreground segmentation masks.
%
We use the image thinning method to extract one pixel wide medial axis curves from $\segI$, which are called {\em skeletal curves} and henceforth denoted by $\skelC=\{\skelCk{k} \subset  \mathbb{R}^2, k=1 \sim \frameNum\}$.
%
%In this way, the input image sequence $\inputI$ is converted into a sequence of images $\thinI=\{\thinIk{k}, k=1 \sim \frameNum\}$ containing one-pixel wide curves.
%
%\james{Many notations defined here are no longer used in the following paragraphs, we should remove those redundant notations...}
%

\subsection{Phase I: Estimation of Camera Poses and Curve Network}
\label{sec:phaseI}
%
%Next we present an 
We develop an optimization framework to simultaneously compute all camera poses and a 3D skeletal curve network.
%
The camera pose of input image $\inputIk{k}$ is parameterized by the respective camera rotation $\camRk{k}$ and translation $\camTk{k}$.
%
%for its rotation and translation relative to some reference frame. 
The 3D curve network $\curveStruct$ of the entire object to be reconstructed is represented as a graph $G=(\mathbf{P},\mathbf{E})$, where $\mathbf{P}=\{p_i \in \mathbb{R}^3, i=1 \sim \curvePntNum\}$ represents a sequence of 3D points appropriately sampled on the 3D curve and the edge set $\mathbf{E}$ encodes the connectivity of the 3D points.
%
%%The network is composed of 3D skeletal curve segments $C_i$, each of which we 
%We will represent each curve segment $C_i$ 
%represent as a sequence of 3D points $p_j$ appropriately sampled on $C_i$. Thus the geometry of the curve network $C$ is represented by the coordinates of all its 3D points. 

% which is in correspondence  and suppose that they are in correspondence with the 2D image curve segments $\overline{C}_{k,i}$ in the view $\overline{I} I_k$
% \begin{equation}
%     F(\{R_k, T_k\}; C) = \sum_{k, i}{\rm dist}^2(\pi (R_k, T_k; C_i), \overline{C}_{k, i}),
%     \label{FF}
% \end{equation}

% \input{figure/fig_formulation.tex}. 

%Our goal now is to define an objective function in terms of the camera poses $(R_k, T_k)$ and the curve geometry $C$ as variables and minimize this objective function to determine the accurate camera poses and the curve geometry to achieve high-quality thin structure reconstruction.
%
We compute the camera poses, $(\camRk{k}, \camTk{k})$, and the curve network, $\curveStruct$, by minimizing an objective function that measures the sum of the squared 2D distances between the projection of the curve network, $\curveStruct$, in an input view $\inputIk{k}$ and the corresponding 2D skeletal curve $\skelCk{k}$, across all input views: 
%an input view $I_k$ and its corresponding 2D image curve $\overline{C}_{k}$ in $\overline{I}_k$, for all the input views $I_k$.  
%
\begin{equation}
    F(\{\camRk{k}, \camTk{k}\}; \curveStruct) = \sum_{k}{\rm dist}^2(\curveProjk{k}, \skelCk{k}),
    \label{eq:obj_function}
\end{equation}
%
where $\curveProjk{k}=\pi (\camRk{k}, \camTk{k}; \curveStruct)$ is the projection of $\curveStruct$ onto view $\inputIk{k}$ using camera extrinsic parameters $(\camRk{k}, \camTk{k})$. 
%We denote this projection by $\overline{C}'_{k,i} = \pi (R_k, T_k; C)$.  Then we define the objective function as
%
Further, ${\rm dist}^2(\curveProjk{k}, \skelCk{k})$ indicates the one-sided integrated squared distance between the curve $\curveProjk{k}$ and the curve $\skelCk{k}$ in the 2D image plane, which is defined as: 
\[
{\rm dist}^2(\curveProjk{k}, \skelCk{k})= \int_{p \in \curveProjk{k}} \min_{q \in \skelCk{k}} \|p-q\|_2^2,
\]
where $\|\cdot \|_2$ is the Euclidean norm.
%
In the following, we explain an iterative scheme to minimize this objective function.
%
Starting from two input images, our method progressively adds input frames one-by-one to a set of active images to estimate $(\camRk{k}, \camTk{k})$, and refines $\curveStruct$ on the currently active image set in an alternating manner.

%at each iteration it computes an estimate of $(R_k, T_k)$ and $C$ on the currently active image set in an alternating manner. In the following, we also describe how to initialize all variables at the beginning.

\subsubsection{Initialization}
\label{sec:initialize}
%
%\james{Need to revise this part...}
%\CT{following is unclear - are the two first frames in what I called above the active image set not always the first two frames of the video ? - so it can also be frame 1 and 10 ?}
%\WP{To be revised by Wenping.}
%\james{We use the first two frames in the current implementation, but can the system still work from arbitrary two frames? Because we didn't have time to do an ablation study on testing initial condition. It is better we just say we always use the first two frame to bootstrap the system.}


Now we discuss how to initialize the camera poses and the 3D curve network in order to solve the optimization problem formulated in~\eqnref{obj_function}.
%
Since a proper initialization will largely facilitate the later incremental reconstruction of thin structure, we propose to select two image frames that meet the criterion of presenting sufficient camera movement such that the resulting parallax could provide sufficient depth information.
%
Specifically, we prepare a sequence of image pairs, denoted as $\{(\inputIk{1}, \inputIk{i}), i=2, 3, \dots \}$ and evaluate the image pairs successively in the following way. 
%
Given an image pair, we compute a pixel-wise correspondence between the curve segments using a 2D curve matching method~\cite{kraevoy:eg:2009} that exploits optical flow~\cite{eccv:kroeger:2016} to estimate an initial coarse alignment between two images.
%
Based on the correspondence induced by the matching curves, we jointly estimate the camera poses of these two frames and a 3D point cloud using the bundle adjustment~\cite{triggs:bundle:1999}.
We then choose the first pair where the distance between two camera locations is larger than $0.03$. Note that the distance is normalized by the average depth of the points relative to the first camera.


%


% Now we discuss how to initialize the camera poses and the 3D curve network in order to solve the optimization problem formulated in~\eqnref{obj_function}.
% %
% Since a proper initialization will largely facilitate the later incremental reconstruction of thin structure, we propose to select two image frames that meet the criterion of presenting sufficient camera movement such that the resulting parallax could provide sufficient depth information.
% %
% Given two input frames, we compute a pixel-wise correspondence between the curve segments using a 2D curve matching method~\cite{kraevoy:eg:2009} that exploits optical flow~\cite{eccv:kroeger:2016} to estimate an initial coarse alignment between two images.
% %
% Then, based on the correspondence induced by the matching curves, we jointly estimate the camera poses of these two frames and a 3D point cloud using the bundle adjustment~\cite{triggs:bundle:1999}.
% %
% Next, we propose a greedy yet effective strategy to select two input frames for initialization.
% %
% First, we prepare a sequence of image pairs, denoted as $\{(\inputIk{1}, \inputIk{i}), i=2, 3, \dots \}$.
% %
% Then we apply the bundle adjustment as described above to the pairs $\{(\inputIk{1}, \inputIk{i})\}$  successively and choose the first pair where the distance between two camera locations is larger than $0.03$. The distance is normalized by the average depth of the points relative to the first camera.


\paragraph{{\bf Curve network generation}}
After the initial 3D point set is generated, we connect the points into a 3D curve network using a variant of Kruskal's algorithm to compute the minimum spanning tree~\cite{kruskal:shortest:1956}.
%
The goal is to build a general curve structure rather than a tree-like structure for representing a wide range of object.  
% the generated curve network shall be allowed to have a general topology, not only a tree-like topology, in order to represent a wide range of objects. 
%
%
The network formation algorithm has the following steps:
%
\begin{enumerate}
\item  Given a set of 3D points, $\mathbf{P}$, we first form a set of candidate edges $\mathbf{E'}$ by pairing points with a mutual distance below 
%distance between the two points less than 
a preset threshold $\theta$, that is, 
$\mathbf{E'} =\{(p_i, p_j) | p_i, p_j \in P,  i\neq j,  \|p_i - p_j \||< \theta )\}$. 
%We experimentally determined $\theta = 5 \delta_0$ to be appropriate, where $\delta_0$ is the sampling distance defined below. 
We empirically set $\theta = 5 \delta_0$, where $\delta_0$ is the sampling distance defined below.
%
\item  A graph $G=(\mathbf{V},\mathbf{E})$ is maintained, with $\mathbf{V}=\mathbf{P}$ and $\mathbf{E}=\emptyset$ (empty set). 
%\item  Consider adding the edges of $\mathbf{E'}$ to $\mathbf{E}$ in the ascending order of the edge length.
\item Check, in ascending order of the edge length, if the edges of $\mathbf{E'}$ shall be added to $\mathbf{E}$.
%in the ascending order of the edge length.
%
%An edge $(p_i, p_j)$ to $E$ i, after adding  $(p_i, p_j)$ to $E$, there does not exist path  $G$ or there is a path in $G$ but the length of this path is greater than threshold $L$, (We set $L = 20$ in our experiment.)
An edge $(p_i, p_j) \in \mathbf{E'}$ is added to $\mathbf{E}$ if it does not form a loop in the graph $G$ or the length of the loop formed by the edge is greater than a threshold $L$. We set $L = 20 \delta_0$ in our experiments, where $\delta_0$ is the sampling distance defined below.
%
\item Repeat step (3) until all edges in $\mathbf{E'}$ have been processed.
\end{enumerate}

However, only loops larger than a minimal size threshold shall be allowed in the curve network in order to avoid the formation of erroneous small loops due to noise in the point cloud.

\paragraph{{\bf Curve re-sampling}}
Since the 3D points in $\mathbf{P}$ that define the geometry of curve network $G$ are directly "lifted" from pixels in an input view, the distribution of the points is in general not uniform.
%
We improve this by re-sampling points on the curve network with an even distribution. 
%
% explain how the curve network is sampled to get its polygonal representation and how this representation is used to find matching curve segments between the curve network and the 2D image curves.
%
We suppose that the center of the object being scanned has unit distance to the camera center. Then the inter-point sampling distance is set to be $\delta_0 = 1/f_0$, where $f_0$ is the camera focus length, which is identical across all the input frames. The rationale for setting the sampling distance in this way is to ensure that, when projected onto the input view, the sample points on the 3D curve have nearly the same density as the image pixels.

Note that both aforementioned steps, curve network generation and curve re-sampling, are performed not only during initialization but also when the points are updated in every iteration of minimizing the objective function defined in~\eqnref{obj_function}.

% First, suppose that a dense point cloud has been reconstructed and connected into a 3D curve network at an initialization step (see Section \ref{sec:initialize}).  This 3D curve is sampled by a sequence points inter-point sampling distance set to be $\delta_0 = 1/f_0$, where $f_0$ is the camera focus length and it is assumed to remains unchanged for all the frames in an input video. 

% \paragraph{Topology refinement} \WP{This is about merging two or more nearby junctions into a single junction. To be cleaned up}. 
% A simple topological graph is not accurate enough for the final structure. Though efficient in the iteration procedure, our variant of spanning tree method usually generates artifacts on multi-to-one junctions due to local ambiguity. \textbg{Figure is needed here, show an 8 to 1 junction and the }. To solve the problem, we conduct a topology refinement on the 3D structure, inspired by the idea of reverse drawing from Noris ~\etal~\shortcite{noris:sigg:2013}. (Do we need to add more details here?) \textbf{ figure here: reverse drawing: 1. remove ambiguous region. 2. Find the position of junction }

\subsubsection{Iterative Camera and Curve Estimation}
\label{sec:iteration}

\paragraph{{\bf Curve matching}}
% \heading{Curve matching} 
%\WP{This is about matching a part of the 3D curve with the correct curve observed in input images. Wang Peng will fill in more  detail, A figure is needed.} 
%
A key step in solving the minimization problem in~\eqnref{obj_function} is our {\em curve matching} step that establishes the correspondence between the points of 3D curve $\curveStruct$ and those on the observed image curves $\skelCk{k}$ in each input image.
%
%The natural but 
A naive distance-based criterion would be finding the closest point $q_j \in \skelCk{k}$ to the projection of any given point $p_j \in \curveStruct$, and set $q_j$ as the matching point of $p_j$.
%
Clearly, this greedy approach may often yield wrong matching points when the observed image curve $\skelCk{k}$ is dense and cluttered (see~\figref{matching}(a)).
%

We solve this problem by combining a distance-based criterion with a constraint on curve consistency, which indicates that two consecutive sample points $\{p_i,p_{i+1} \in \curveStruct\}$ should have their corresponding points $\{q_j,q_{j+1}\}$ lie on the same local branch of the image curve $\skelCk{k}$ and be close to each other (see~\figref{matching}(b,c)).
%
%\james{Figure 3 does not clearly illustrate what we want to say...}

%Specifically, suppose that the 3D curve $\curveStruct$ is represented by the point sequence $P$ = $\{p_j\}_{j=1}^N$ and the image curve $\overline{C}_k$ in $I_k$ be represented by the pixel sequence $Q_k = \{q_i\}_{i=1}^h$. A matching of $C$ with $\overline{C}_K$ is then defined by an injection $\phi$ from $[1, N]$ into $[1, K]$. Let $\Phi$ denote the set of all such injections, Then we seek the optimal matching $\phi_0$ that minimizes the follow functional
%
Specifically, suppose the 3D curve $\curveStruct$ is represented by the point sequence $\mathbf{P}=\{p_i \in \mathbb{R}^3, i=1 \sim \curvePntNum\}$ and the observed image curve $\skelCk{k}$ in the image $\inputIk{k}$ is represented by the pixel sequence $\mathbf{Q}=\{q_i \in \mathbb{R}^2, i=1 \sim \skelPntNum\}$. A matching between $\mathbf{P}$ and $\mathbf{Q}$ is then defined by an injection $\phi$ from $[1, \curvePntNum]$ into $[1, \skelPntNum]$. Let $\Phi$ denote the set of all such injections. Then we seek the optimal matching $\phi_0$ that minimizes an objective function defined as follows:
%
\begin{equation}
\begin{aligned}
E_{match} (\curveStruct, \skelCk{k}) = \alpha \sum_{j} \|\pi (p_j) - q_{\phi(j)}\| + \\ \sum_{j} \|(\pi(p_j) - \pi(p_{j+1})) - (q_{\phi(j)} - q_{\phi(j+1)})\|.
\end{aligned}
\end{equation}
%
We empirically set $\alpha=0.1$ in our experiments.
This minimization problem is solved efficiently with dynamic programming. %Given a point $p_j$, we consider its candidate matching points $q_i$ only in the local neighborhood with radius $10$ pixels of the projection point $\pi (p_i)$. \WP{Wang Peng, please add a figure here (Figure to add)}.
Given a point $p_i \in \curveStruct$, we select the candidates for $p_j$'s matching points only among those pixels $q_j \in \skelCk{k}$ lying within a circle of radius of $10$ pixels centered at the projected point $\pi (p_i)$.



% by neighborhood searching around $\pi(p_i^j)$ (with radius = 10 pixels in our experiments), we optimize the path-level selection problem by dynamic programming.
% % Given any input view $I_k$, for each segment $C_i$ of the 3D curve network $C$, it is critical to find the correct marching image curve $\overline{C}_{k,i}$ of the projection $\overline{C}'_{k,i}$ of  $C_i$ onto the image plane of $\overline{C}$. .....
% % % Wang Peng's description
% % \par
% We now describe our 3D curve to 2D curve points matching algorithm. 
% For 3D curve segment $C_i$, and image view $I_k$, assume that its sampled points sequence is $P_i$ = $\{p_i^1, p_i^2,...,p_i^n\}$ and we need to find optimal correspondences described as 2D point sequence $Q_k = \{q_k^1, q_k^2,...,q_k^n\}$ between $S_i$ and $I_k$. Considering both local distance cost and global smoothness, we would like to optimize such function :
% \begin{equation}
% S(C_i, Q_k) = \alpha \sum_{j}^{}{|\pi (p_i^j) - q_k^j|} + \sum_{j}^{}{|(\pi(p_i^j) - \pi(p_i^{j+1})) - (q_k^j - q_k^{j+1})|}
% \end{equation}


\input{figure/fig_matching.tex}

\paragraph{\bf{Optimization strategy}}
There are two sets of variables in the objective function (see~\eqnref{obj_function}): (1) the camera pose parameters $(\camRk{k}, \camTk{k})$ and (2) the sample points of the curve network $\curveStruct$.
%
To simplify the optimization task, we process the camera poses in a progressive manner so that a new camera view is added after the camera poses of all the preceding views have been estimated. 
%
Similarly, the curve network is also refined in a progressive manner since, in general, new curve geometry may be captured and recovered in other video frames. 

Based on the discrete representation of the curve network, we can rewrite the~\eqnref{obj_function} as:
%
\begin{equation}
    \resizebox{0.9\hsize}{!}{
    \tilde F(\{\camRk{k}, \camTk{k}\}; \curveStruct) = \sum_{k}  \sum_{p_j \in \curveStruct} \occluFunc(p_j, \inputIk{k}) \cdot \min_{q \in \skelCk{k}} \|\pi (\camRk{k}p_j + \camTk{k}) - q\|_2^2,
    }
    %\label{FD}
    \label{eq:obj_function_discrete}
\end{equation}
%
where the distance error term
%
\begin{equation}
    e_{k,j} \equiv \min_{q \in \skelCk{k}} \|\pi (\camRk{k}p_j + \camTk{k}) - q\|_2^2
    %\label{de}
    \label{eq:dist_error}
\end{equation}
%
is the squared distance from the projection of a variable point, denoted as $p'_j = \pi (\camRk{k}p_j + \camTk{k})$, to the observed image curve $\skelCk{k}$.
%
And $\occluFunc(p_j, \inputIk{k})$ is an indicator function that returns value 0 if the point $p_j$ fails to pass the self-occlusion test with respect to the input view $\inputIk{k}$, and otherwise returns value 1.
%
The details of self-occlusion handling process are elaborated in~\secref{occlusion}.

\input{figure/fig_error_term.tex} 

\input{figure/fig_self_occlusion.tex}

\input{figure/fig_visual_results.tex}


In practice, we adopt a commonly used formulation for curve fitting~\cite{pottmann:CGA:2002} to efficiently minimize the distance error term $e_{k,j}$ in~\eqnref{dist_error} by expressing it as a special linear combination of the squared distances of $p'_j$ to the image curve $\skelCk{k}$ along the normal direction, $n_j$, and tangent direction, $t_j$, at the corresponding point $q_j \in \skelCk{k}$ (see~\figref{error_term}).
%
Thus, by denoting $v_j = \pi (\camRk{k}p_j + \camTk{k}) - q_j$, \eqnref{obj_function_discrete} can be further expressed as
%
\begin{equation}
\resizebox{0.9\hsize}{!}{
    \tilde F^* (\{\camRk{k}, \camTk{k}\}; \curveStruct) = \sum_{k}  \sum_{p_j \in \curveStruct} \occluFunc(p_j, \inputIk{k}) \cdot \left[{}\| v_j \cdot n_j \|^2 + w \| v_j \cdot t_j\|^2 \right]  +  F_s(C),
    }
    \label{eq:obj_function_final}
\end{equation}
%
where $F_s(C)$ is a regularization term defined as follows:  
$$F_s(C) = \lambda \sum_{k}  \sum_{p_j \in \curveStruct} \| p_{j+1} - 2 p_j + p_{j-1}\|^2. $$
%
We set the weight parameter $\lambda = (\frac{2.5}{\sigma_0})^2$ and $w$ with value $0.5$ in our experiments for a trade-off between efficiency and stability of convergence.

%\paragraph{Optimization strategy}
We minimize the objective function $\tilde F^*$ iteratively. 
In each iteration, $\tilde F^*$ is minimized in an alternating fashion that first optimizes the camera poses $\{(\camRk{k}, \camTk{k})\}$ while fixing the curve points $\{p_j\}$, and then optimizes the curve points while fixing the camera poses. The process iterates until the curve points stop moving.
%
Note that, once the camera poses $\{(\camRk{k}, \camTk{k})\}$ and the points $\{p_j\}$ have been updated, we re-compute the corresponding point $q_j$ on the image curve $\skelCk{k}$ to the updated projected point $p'_j$ by our matching algorithm before entering the next iteration.

% ====== commented out by James =======
% \begin{comment}
% At any time of optimization, suppose we have the camera poses of the first $m$ views, represented by the parameters $P_m = \{ (R_k, T_k) \}_{k=1}^m$ and the current observable curve network $C$, which is represented by the points $\{p_j\}_{i=1}^n$. Based on this discrete representation of the curve $C$, denoting the projection of $p_j$ into the view $I_k$ by $\bar p_j = \pi (R_k p_j + T_k)$, we approximate the objective function $F$ in Eqn. (\ref{FF}) by the following function
% \begin{equation}
%     \tilde F(\{R_k, T_k\}; C) = \sum_{k}  \sum_{p_j \in C} NSC(p_j, I_k) \cdot \min_{q \in \overline{C}} \|\pi (R_kp_j + T_k) -q\|_2^2,
%     \label{FD}
% \end{equation}
% where the distance error term 
% \begin{equation}
% e_{k,j} \equiv \min_{q \in \overline{C}} \|\pi (R_kp_j + T_k) -q\|_2^2
% \label{de}
% \end{equation}
% is the squared distance function from the variable projection point $\bar p'_j = \pi (R_kp_j + T_k)$ to the image curve $\overline{C}$. Here $NSC(p_j, I_k)$ is a function taking values 0 or 1, used to indicated the self-occlusion status of $p_j$ with respect to the input view $I_k$.  When the point $p_j$ is {\em not} involved in self-occlusion with respect to $I_k$, we have $NSC(p_j, I_k) = 1$ and then the term $e_{k,j}$ in included the function $\tilde F$; $p_j$ is involved in self-occlusion with respect to $I_k$, we have $NSC(p_j, I_k) = 0$ and then $e_{k,j}$ in included, The evaluation of the function $NSC(p_j, I_k)$ is detailed later in Section \ref{sec:occlusion}.

% This objective function in Eqn. (\ref{FD}) is commonly used for curve fitting~\cite{pottmann:CGA:2002}, where it is suggested that an efficient way for minimizing the distance error term $e_{k,j}$ in Eqn. (\ref{de}) is to express it as a special linear combination of the distances of $p'_j$ to the curve $\overline{C}$ along the normal direction and the tangent direction of the curve $\overline{C}$ at $q$, respectively. Specifically, suppose that $(R_k, T_k)$ and the points $p_j \in C$ are fixed at the moment. Let $q_j \in \overline{C}_{k,i}$ be the closest point on $\overline{C}_{k}$ to the point $p'_j = \pi (R_kp_j + T_k)$. Let $t_j$ and $n_j$ be the unit tangent vector and unit normal vector of the curve $\overline{C}_{k}$ at $q_j$, respective. 
% \input{figure/fig_error_term.tex} 
% \LJ{A figure is needed here} \WP{Wang Peng, could you add an illustrative figure here?}
% Denote $v_j = \pi (R_kp_j + T_k) - q_j$. 
% Then, following~\shortcite{pottmann:CGA:2002}, the function $\tilde F(\{R_k, T_k\}; C)$ is approximated by 
% \begin{equation}
%     \tilde F^* (\{R_k, T_k\}; C) = \sum_{k}  \sum_{p_j \in C} \left[{}\| v_j \cdot n_j \|^2 + w \| v_j \cdot t_j\|^2 + f_s(p_j) \right]
%     \label{FD}
% \end{equation}
% where $f_s(p_j)$ is a regularization term defined by  
% $$f_s(p_j) = \| p_{j+1} - 2 p_j + p_{j-1}\|^2. $$
% Here $w = 0.5$ is used in our experiments for trade-off between efficiency and stability of convergence. 
% 
% In each iteration, the function $ \tilde F^*$ is minimized alternatively with respect to the variable camera poses $\{(R_k, T_k)\}$ while fixing the points $\{p_j\}$, and then with respect to the variable points $\{p_j\}$ while fixing the camera poses $\{(R_k, T_k)\}$. Note that, once the camera poses $\{(R_k, T_k)\}$ and the points $\{p_j\}$ have been updated, we need to re-compute the closest point $q_j$ on the image curve $\overline{C}_{k}$ to the updated projection point $p'_j = \pi (R_kp_j + T_k)$ before entering the next iteration of minimizing $\tilde F^*$ in Eqn. (\ref{FD}).
% \end{comment}
% The detailed computation of the radius function will be discussed shortly. 

\subsubsection{Handling Self-occlusion} 
\label{sec:occlusion}

A {\em self-occlusion} occurs when distinct parts of a 3D curve network $\curveStruct$ are projected onto the same location in a 2D view $\inputIk{k}$. 
%
When this happens, the 3D curve $\curveStruct$ intersects itself in the projected view where the intersecting pixels correspond to multiple points of $\curveStruct$, causing ambiguity during the reconstruction (see~\figref{self_occlusion}(a)).
%
Hence, it is critical to detect self-occlusion to ensure that image observations involving self-occlusion are not used for 3D curve reconstruction. 

To determine whether the points of 3D curve $\curveStruct$ are subject to self-occlusion in a certain image $\inputIk{k}$, we perform the following steps:
%
\begin{enumerate}
\item For each point $p_j \in \curveStruct$ and its matching point $q_{\phi(j)} \in \skelCk{k}$ paired in the curve matching step, we examine the neighboring pixels of $q_{\phi(j)}$ using a $3 \times 3$ local window. We then generate a 3D point set $\hat{\mathbf{P}}$ that contains whatever points of $\curveStruct$ that match the pixels within the local window.
%
\item We then compute a spatial compactness factor as the standard deviation $\sigma_j$ derived from the L2 distance between the points in $\hat{\mathbf{P}}$ and their centroid.
%
\item Point $p_j$ is labeled as self-occluded (\ie $\occluFunc(p_j, \inputIk{k})=0$) if $\sigma_j \geq \sigma_0$. Otherwise if $\sigma < \sigma_0$ and all the points in $\hat{\mathbf{P}}$ lie on the same local branch of the 3D curve $\curveStruct$, the point is not self-occluded (\ie $\occluFunc(p_j, \inputIk{k})=1$).
%
\end{enumerate}
%
We use a preset threshold $\sigma_0=10 \delta_0$ in our experiments. 
%
We employ this self-occlusion handling not only during the 3D curve reconstruction but also during the surface reconstruction in Phase II in order to obtain reliable radius estimates as discussed below.


% ====== commented out by James =======
% \begin{comment}
% {\em Self-occlusion} refers to that two or more parts of a 3D curve network $\curveStruct$ with different depths are projected to the some location in a 2D view $I_k$. When this happens, the 2D projection curve $\skelCk{k}$ of the 3D curve $C$ intersects itself and the intersection point $q_0 \in \skelCk{k}$ corresponds to multiple points of $\curveStruct$, causing ambiguity to reconstruction. Hence, it is critical to detect self-occlusion to ensure that image observations involving self-occlusion are not used for 3D curve reconstruction. 

% Our method for detecting self-occlusion work as follows. First, an indicative function $NSC(p_j, I_k)$ is defined. Here $NSC(p_j, I_k) = 1$ means that the point $p_j$ on the 3D curve $C$ is not involved in self-occlusion with respect to the input view $I_k$; otherwise, if $NSC(p_j, I_k) = 0$, there is self-occlusion involving $p_j$ with respect to $I_k$.

% To efficiently evaluate $NSC(p_j, I_k)$ for all the sample points $p_j$ of $C$ and all the input views $I_k$, we examine the $3\times 3$ neighborhood of each pixel $q$ on the image curve in $I_k$, denoted by $\tilde N(q)$. 
% %
% We then compute the standard deviation $\sigma$ of the distances of the points in $\tilde N(q)$ to their geometric centroid. The rationale of measuring $\sigma$ is that, if there is self-occlusion occurring at the pixel $q$, the points of $\tilde N(q)$ should come from different curve branches of $C$ so should be apart from each other, thus giving rise to a large standard deviation $\sigma$. Hence, we set $NSC (pi, I_k) :=0$ for all the points $p_j$ in $\tilde N(q)$ if $\sigma \geq \sigma_0$ for a pre-specified threshold $\sigma_0$, because a large $\sigma$ implies the likelihood of self-occlusion. Otherwise, if $\sigma < \sigma_0$ and that the points $\tilde N(q)$ all lie on the same local branch of the curve $C$, then we set $NSC (p_j, I_k) := 1$ for all the points $p_j$ in $\tilde N(q)$, meaning no self-occlusion. In this way, $NSC (p_j, I_k)$ is evaluated for all the points $p_i \in C$ after checking all the images curve pixels in all the input views. 

% Self-occlusion detection allows us to ensure that only reliable image observation not involving self-occlusion is used for constructing the 3D  curve network and estimating the radius of the thin structure. When a point $p_j \in C$ needs to be updated by minimizing the objective function $\tilde F$ in Eqn. (\ref{FD}), its associated error term $e_{k,j}$ (Eqn. (\ref{de})) is included in the objective function $\tilde F$ only if $NSC(p_j, I_k) = 1$. Similarly, when estimating the radius of the thin structure at the point $p_j$, the observation from the image $I_k$ should be used only if $NSC(p_j, I_k) = 1$. 
% \end{comment}




% This ambiguity of one-to-many correspondence, the image observation at $q_0$ should not be used for 3D curve network reconstruction. 
% that is, . Self-occlusion of a 3D curve is not a local property, because it depends on the global structure of the curve as well as a particular viewing perspective. Self-occlusion occurs frequently and causes ambiguity to 3D reconstruction because the intersection point in the image corresponds to more than point on the 3D curve. If a part of a 2D image curve is found to contain self-occlusion, then that part of curve should be excluded from consideration for 3D reconstruction. So it is important to detect self-occlusion for high quality reconstruction. \WP{Wang Peng, please add an illustrative figure here, showing a 3D curve segment projecting to a self-intersecting 3D curve.}  

% would provide unreliable information about the corresponding 3D curve so should be excluded from consideration in order to make the reconstruction process more robust. Self-occlusion is a main reasons why it is more challenging to reconstruct a wire model than a general object using an image-based or video-based method.  If a part of a 2D image curve is detected to contain a self-occlusion point, then that part of the curve would provide unreliable information about the corresponding 3D curve so should be excluded from consideration in order to make the reconstruction process more robust. In the following we will explain how to detect self-occlusion and how the detection results is used to improve the performance of our reconstruction pipeline. 
% We have developed an effective technique for determining whether a part of the 3D curve network is involved in self-occlusion. 

% associate a self-occlusion label function $SC (p_j, I_k)$ to each sample point $p_j$ of the 3D curve network $C$ relative the input image $I_k$. Here $SC (p_j, I_k) =TRUE$ means $p_j$ is involved in self-occlusion with respect to the view $I_k$. 
% To evaluate $SC (p_j, I_k)$ for all the points $p_j$ of $C$ with respect to all the input images $I_k$, we perform the following searching procedure for all the 2D pixel curves in all the input images. For any point $q$ on the image curve $\overline{C}_k$ in the view $I_k$, let $N(q, d)$ denote the $d\times d$ neighborhood of pixels centered at $q$ (we take $d=3$ in our implementation).
% % denote the set of $q$'s neighboring pixels on $\overline{C}_k$ whose distances to $q$ are at most $d$, assuming that the width of a pixel is 1. \WP{(We set d=2 in all our tests.)} % define $N(q; d) = \{u \| |u - q| \leq d, u\in C'_k u \}$, 
% We then find all the sample points on the 3D curve $C$ that are projected into the set $N(q; d)$, and denote these points by $\tilde N(q)$. 


\subsection{Phase II: Surface Geometry Reconstruction}
\label{sec:surf_reconstruct}
%
To generate the generalized cylinder (or sweep surface) representing the surface of the reconstructed thin structure, we compute the radius at each point of the 3D curve using the corresponding image observations from all the input views.
%
Specifically, for each point $p_j$ of 3D curve $\curveStruct$, we first find its matching point $q_{\phi(j)} \in \skelCk{k}$. 
%
Note that the projection of a generalized cylinder is a 2D strip in an input image.
%
Therefore we compute the width of the strip at the point $q_{\phi(j)}$ by computing the distances from $q_{\phi(j)}$ to both sides of the strip defined in the foreground segmentation mask $\segIk{k}$. We denote the estimated width by $2\bar{r}_j^k$ (see~\figref{self_occlusion}(b)).
%
Then the radius of the thin structure at $p_j$ in the image view $\inputIk{k}$ is defined as:
%
\begin{equation}
r_j^k = \frac{\bar{r}_j^k}{f_0} \times {\rm depth}(p_j, \inputIk{k}),
\end{equation}
%
where $f_0$ is the focal length of the camera and ${\rm depth}(p_j, \inputIk{k})$ is the depth of $p_j$ with respect to the image $\inputIk{k}$.
%
The final estimated radius at $p_j$ is thus defined as the average of the $r_j^k$ over all the input images, excluding those image observations that involve self-occlusion at $p_j$, \ie $\occluFunc(p_j, \inputIk{k})=0$.

% % ====== commented out by James =======
% \begin{comment}
% To generate the generalized cylinder (or sweep surface) representing the thin structure, we compute the radius at each point of the 3D curve from the projection of the thin structures in the input views.
% %
% Specifically, for each point $p_j$ of 3D curve $\curveStruct$, we first find $q_j^k$ on the image curve in image $I_k$. Note that the projection of a generalized cylinder is a 2D strip in an input image, barring self-occlusion. Then we find the width of the strip at the point $q_j^k$ by computing the distances from $q_j^k$ to both sides of the strip. Let this width be denoted by $\overline{r}_j^k$ (see~\figref{??}) \WP{Add a figure of a 2D strip here with notation about its width?}. Then the radius of the thin structure at $p_j$ as estimated from the view $I_k$ is given by
% %
% \begin{equation}
% r_j^k = \frac{\overline{r}_j^k}{f_0} \times {\rm depth}(p_j, I_k)
% \end{equation}
% %
% where $f_0$ is the focal length of the camera and ${\rm depth}(p_j, I_k)$ is the depth of $p_j$ with respect to the image $I_k$. Then we set the radius at $p_j$ to be the average of the $r_j^k $ over all the input images $\{I_k\}{i=1}^m$ that do not contain self-occlusion involving the point $p_j$, that is, image observations that might be contaminated by self-occlusion are not used for radius estimation. The details of detecting self-occlusion are given in the next section. 

% % In ideal situations, to obtain the 3D radius of point $p_j$, we can fuse the the radius information from all the camera views by simply averaging them. However, due to the occlusion (WangPeng: figure is needed here.), the 2D radius estimation from some camera views could be quite inaccurate. Thus, we restrain the occlusion by the strategy introduced in \ref{sec:occlusion} and only consider the radius information of image $I_k$ with $SC(P_j, I_k) = FALSE$.
% \end{comment}





==> 7_acknowledgements.tex <==

\section{Acknowledgements}
%\begin{comment}
%\hl{
We would like to thank the reviewers for their valuable and insightful comments. We also thank Shiwei Li, Amy Tabb, Rhaleb Zayer for their help with experiments. This work was partially funded by the Research Grant Council of Hong Kong (GRF 17210718), ERC Consolidator Grant 770784, Lise Meitner Postdoctoral Fellowship, Ministry of Science and Technology of Taiwan (108-2218-E-007-050 and 107-2221-E-007-088-MY3).
%}
% \end{comment}
\label{sec:acknowledgements}

==> backup/3_back_overview.tex <==
\section{Method}
\label{sec:method}
% ================================================================
% What is the input and output of the system?
% Define the notation if necessary
% ================================================================

\subsection{Overview}
Given a physical 3D thin structure (or wire model), our goal is to reconstruct the model, i.e. obtaining its 3D digital representation, from a 2D video sequence. It is assumed that the intrinsic parameters of the camera taking the input video are known and fixed, but the motion (or poses) of the camera is unknown. 

Similar to [Wire Art] and [Curve Fusion], we define a thin structure as a collection of connected generalized cylinders, where each generalized cylinder sweep surface of varying radius along its {\em skeletal curve}. Therefore, we represent a thin structure as a network of connected skeletal curves, to be called the {\em curve network} for short, with a radius function defined on the skeletal curves. We will elaborate later how to convert a point cloud reconstructed from the image observation into such a curve network. In our algorithm, the network of the skeletal curves is first reconstructed \revised{(~\secref{optimize})} and then the radius function is estimated from image observation to recover the surface geometry of the thin structure \revised{(~\secref{surf_reconstruct})}. The reconstruction quality is measured by the accuracy of the skeletal curves and the radius function, as well as whether the joints of the curve network are correctly recovered.

Finding correspondence of the features between different images is key to reconstructing a 3D object from multiple images or video (i.e. an ordered sequence of images). When the camera poses are known, the task of finding corresponding image points is facilitated by using epipolar constraints between different images. In our setting, since the camera poses are unknown, we use spatial coherence among the image frames of the input video to efficiently search for image point correspondence. 
%Furthermore, due to the lack of point features on thin structures, we rely on the matching between skeletal curve segments, instead of point features, to establish the correspondence between two images. 
\revised{Furthermore, due to the textureless natural of the thin structure, we rely on the matching between skeletal curve segments to establish the point correspondence between to images.} 

Now we outline our strategy to recover both unknown camera poses and the unknown geometry of the curve network \revised{(~\secref{optimize})}. At any stage, we maintain the estimated values of the following two sets of valuables: extrinsic parameters defining the poses of the camera and the set of 3D points defining the curve network. After a proper initialization step, which will be explained later \revised{in~\secref{initialize}}, we use an iterative optimization strategy to compute the accurate values of these variables by minimizing the difference between the projection of the curve network and their corresponding image curves in all input image frames \revised{(~\secref{iteration})}. In this process, the image frames (or views) of the input video are added and processed in a progressive manner, and the structure of the 3D skeletal curve network is also improved gradually as more input views are taken into consideration. In the subsequent sections we will present the details of our method and present validation and comparison results to demonstrate its superiority to the existing methods for thin structure reconstruction. 
\james{We miss a key contribution here: how the curvilinear characteristics of the thin structure are exploited to facilitate i) establishing the point correspondence when estimating camera pose (Wang Peng solves an optimization problem there), and 2) also dealing with occlusion issue when updating the point cloud.}

%We denote the reconstructed thin structure as a skeleton curve, $C=(V,E)$, where $V=\{\curvePnt_{i} \in \mathbb{R}^3\}^M_{i=1}$ is the vertices set and $e_{i,j} \in E$ indicates two vertices $\curvePnt_{i}$ and $\curvePnt_{j}$ are connected.  
% %
% \figref{overview} illustrates the overview of our method, which consists of \red{4} stages, including
% \begin{inparaenum}[1)]
% \item {\em preprocessing},
% \item {\em initialization}, 
% \item {\em incremental structure optimization}, and 
% \item {\em surface reconstruction}.
% \end{inparaenum}
% %

% ================================================================
% Describe briefly what each system component does
% Define the notations if necessary
% ================================================================
% %\paragraph{Preprocessing and assumptions.}
% In the preprocessing stage, we first subtract the background image from input images to obtain binary masks of the foreground model at each frame.
% %
% While there are several advanced automatic background subtraction methods~\cite{}, handling foreground models with thin structure remains a challenging task.
% %
% Therefore, we assume that the model is captured in a controlled environment where the background has monotonic color/texture with proper contrast to the foreground.
% %
% The background subtraction is simply carried out via a conventional color keying method or commercial tools (\eg \red{Adobe Affter Effects~\cite{}}).
% %
% Then we apply an image thinning method~\cite{x} to the binary masks to extract a sequence of one-pixel-width 2D skeleton curves (see~\figref{overview}~(a))). 
%
%in which we compute a tangent direction and thickness for each pixel (see~\figref{overview}~(a), \secref{preprocess}).
%




%\end{comment}

==> backup/4_back_method.tex <==
The pipeline of our method include the following key steps, as shown in~\figref{overview}:
\begin{enumerate}
\item {\em Preprocessing for image segmentation \revised{(~\secref{preprocess})}};
\item {\em Initialization of camera poses and a point cloud on the skeletal curves, and connecting the point cloud into a 3D curve network \revised{(~\secref{initialize})};}
\item {\em Iterative optimization to improve the camera poses and the skeletal curve network \revised{(~\secref{iteration})}};
\item {\em Estimating the radius function to recover the surface of the thin structure \revised{(~\secref{surf_reconstruct})}}.
\end{enumerate}

% In this we will present the details of our method and present validation and comparison results to demonstrate its superiority to the existing methods for thin structure reconstruction. 
% (1) variable initialization; (2) connecting the reconstructed point cloud into a 3D curve network; (3) iterative optimization to compute camera poses and 3D curve network; and (4) estimating the radius of the thin structure. 
% \figref{overview} illustrates the overview of our method, which consists of \red{4} stages, including

% Given segmented image $I^k$, we first apply thinning method to get new image $I^{k*}$ with one-pixel width curves. After thinning, for every pixel $p_i$ of $I^{k*}$ with value 1, we estimate its corresponding tangent vector through local weighted PCA: $$M_i^k \in \mathbb{R}^{2\times 2} = \sum_{x,y}{we^{-(x^2 + y^2)}I^{k*}_{p_i}[x,y]^\top[x,y]}$$ is computed and we get eigenvalues $\{\lambda^0, \lambda^2\}$ and eigenvectors $\{v^0, v^1\}$. $v^1$ is regarded as the tangent estimation of pixel $p_i$, and $s_i = \frac{\lambda^2}{\lambda^1 + \lambda^2}$ is the confidence of the tangent vector, indicating how "straight" this region is.

\subsection{Preprocessing}
\label{sec:preprocess}

As a preprocessing step we first segment each input image to obtain a binary mask of the pixels lying on the thin structure. While there exist automatic image segmentation methods~\cite{}, reliable segmentation of thin structures from a general background remains a challenging task. Hence, we assume in this paper that the 3D thin structure is videoed with a simple or clean background so it can be segmented easily using the commonly used color keying method in some commercial tools, \eg Adobe After Effects~\cite{adobe:AE}. Let $\{I_k\}$ denote the input video as a sequence of 2D RGB images. Let $\{I'_k\}$ denote the corresponding image of the segmented binary mark covered by the thin structure. Then we apply a thinning method~\cite{x} to $\{I'_k\}$ to extract one-pixel-width medial axis curves, or called {\em skeletal curves} and denoted by $\bar C_k$, with the resulting image denoted by $\{\bar I_k\}$. In this way, the input video sequence $\{I'_k\}$  is converted into a sequence of images $\{\bar I_k\}$ containing one-pixel-width curves. 

% the background has monotonic color/texture with proper contrast to the foreground.
% %
% The background subtraction is simply carried out via a conventional color keying method or commercial tools (\eg \red{Adobe After Effects~\cite{}}).

\subsection{Formulation of optimization}
\label{sec:optimize}

Next we present an optimization framework for computing the camera poses and the 3D skeletal curve network. Let camera pose of the input image $I_k$ be denoted by the pair $(R_k, T_k)$ for its rotation and translation relative to some reference frame. Let $C$ denote the 3D curve network to be constructed, which is composed of 3D skeletal curve segments $C_i$. We will represent the curve segment $C_i$ as a sequence of points $p_j$ appropriately sampled on $C_i$. Thus the geometry of $C_i$ is presented by the coordinates of the points $p_j$. 

Our goal next is to define an objective function in terms of the camera poses $(R_k, T_k)$ and the curve geometry $C_i$ as variables and minimize this objective function to determine the accurate camera poses and the curve geometry to achieve high-quality thin structure reconstruction. Specifically, our objective function is defined as the sum of the squared distances between the projections of the curve network onto an input view $I_k$ and their corresponding 2D image curves $C_{k}$ in $\bar I_k$, for all the input views $I_k$. Suppose that the 3D curve segments $C_i$ are projected into 2D curve segments $\bar C'_{k,i}$ in the view of $\bar I_k$. Then we denote this projection operation by $\bar C'_{k,i} = \pi (R_k, T_k; C_i)$ and suppose that they are in correspondence with the 2D image curve segments $\bar C_{k,i}$ in the view $\bar I_k$.  \LJ{A figure is needed here} Then we define the objective function as
\begin{equation}
    F(\{R_k, T_k\}; C) = \sum_{k, i}{\rm dist}^2(\pi (R_k, T_k; C_i), \bar C_{k, i}),
    \label{FF}
\end{equation}
where ${\rm dist}^2(\bar C_1, \bar C_2)$ is the one-sided integrated squared distance from the curve $\bar C_1$ to the curve $\bar C_2$ in the 2D image plane, defined as  
\[
{\rm dist}^2(\bar C_1, \bar C_2)= \int_{p\in \bar C_1} \min_{q \in \bar C_2} \|p-q\|_2^2,
\]
where $\|\cdot \|_2$ is the Euclidean norm. In the following we will present our iterative scheme to minimize this objective function, as well as the necessary step for initializing the variables. 

\subsection{Iterative Optimization}
\label{sec:iteration}

There are two sets of variables to solve for in the minimization of the objective function in Eqn. (\ref{FF}): the camera pose parameters $\{R_k, T_k\}$ and the points that define the curve network $C$. To simplify the optimization task, we process the camera poses in a progressive manner so that a new camera view is added only after the camera poses of all the preceding views have been computed. Similarly, the curve network is also reconstructed in a progressive manner since, in general, new curve geometry may be captured by additional video frames. 

At any time of optimization, suppose we have the camera poses of the first $m$ views, represented by the parameters $P_m = \{ (R_k, T_K) \}_{k=1}^m$ and the current observable curve network $C = \{ C_i \}$, where each curve segment is represented by a point sequence $\{p_j\}$. Due to this discrete sampling of the curve $C_i$, noting that the projection of the point $p_j$ into the view $I_k$ is $\bar p_j = \pi (R_k p_i + T_k)$, we may approximate the objective function in Eqn. (\ref{FF}) by the following function
\begin{equation}
    \tilde F(\{R_k, T_k\}; C) = \sum_{k, i}  \sum_{p_j \in C_i} \min_{q \in \bar C_i} \|\pi (R_kp_j + T_k) -q\|_2^2,
    \label{FD}
\end{equation}
where the distance error term 
\begin{equation}
e_{k,j} \equiv \min_{q \in \bar C_i} \|\pi (R_kp_j + T_k) -q\|_2^2
\label{de}
\end{equation}
is the squared distance function from the variable projection point $p'_j = \pi (R_kp_j + T_k)$ to the image curve $\bar C_i$.

This objective function in Eqn. (\ref{FD}) is commonly used for curve fitting as discussed in [{\em cite Pottmann's paper on curve fitting. Ask Wenping.}], where it is suggested that an efficient way for minimizing the distance error term 
$e_j$ in Eqn. (\ref{de}) is to express it as a special linear combination of the distances of $p'_j$ to the curve $\bar C_i$ along the normal direction and the tangent direction at the point $q$ on $\bar C_i$, respectively. Specifically, suppose that $(R_k, T_k)$ and the points $p_j \in C_i$ are fixed at the moment. Let $q_j \in \bar C_{k,i}$ be the closest point on $\bar C_{k,i}$ to the point $p'_j = \pi (R_kp_j + T_k)$. Let $t_j$ be the unit tangent vector of the curve $\bar C_{k,i}$ at $q_j$. \LJ{A figure is needed here}
Denote $v_j = \pi (R_kp_j + T_k) - q_j$. 
Then, following [{\em Pottmann's paper on curve fitting}], the function $\tilde F(\{R_k, T_k\}; C)$ is approximated by 
\begin{equation}
    \tilde F^* (\{R_k, T_k\}; C) = \sum_{k, i}  \sum_{p_j \in C_i} \left[{}\| v_j \times t_j \|^2 + w \| v_j \cdot t_j\|^2 + f_s(p_j) \right]
    \label{FD}
\end{equation}
where $f_s(p_j)$ is a regularization term defined by  
$$f_s(p_j) = \| p_{j+1} - 2 p_j + p_{j-1}\|^2. $$
Here $w = 0.5$ is used in our experiments for trade-off between efficiency and stability of convergence. 

In each iteration, the function $ \tilde F^*$ is minimized alternatively with respect to the variable camera poses $\{(R_k, T_k)\}$ while fixing the points $\{p_j\}$, and then with respect to the variable points $\{p_j\}$ while fixing the camera poses $\{(R_k, T_k)\}$. Note that, once the camera poses $\{(R_k, T_k)\}$ and the points $\{p_j\}$ have been updated, we need to re-compute the closest point $q_j$ on the image curve $\bar C_{k,i}$ to the updated projection point $p'_j = \pi (R_kp_j + T_k)$ before entering the next iteration of minimizing $\tilde F^*$ in Eqn. (\ref{FD}).

\james{Wang peng uses a 2D thickness estimation function in Equation 4 to account for potential occlusion in the view.}

\LJ{STOPPED HERE.}

\subsection{Handling self-occlusion} 
\label{sec:occlusion}

{\em Self-occlusion} refers to the phenomenon that a 3D wire model occludes itself in a 2D view. When this happens, the 2D projection curve of the 3D wire intersects itself, causing ambiguity to 3D reconstruction. Self-occlusion occurs frequently for a complex thin structure and is a main reasons why it is more challenging to reconstruct a wire model than a general object using an image-based or video-based method. If a part of a 2D image curve is detected to contain a self-occlusion point, then that part of the curve would provide unreliable information about the corresponding 3D curve so should be excluded from consideration. Therefore it is critical to detect self-occlusion to make 3D reconstruction robust to its presence. 
In the following we will explain how to detect self-occlusion and how the detection results is used to improve the performance of our reconstruction pipeline. 

We now present an efficient method for determining whether a part of the 3D curve network is involved in self-occlusion.  Self-occlusion of a 3D curve is not a local property, because it depends on the global structure of the curve as well as a particular viewing perspective. The main idea of our method is to associate a self-occlusion label function $SC (p_j, I_k)$ to each sample point $p_j$ of the 3D curve network $C$ relative the input image $I_k$. Here $SC (p_j, I_k) =TRUE$ means $p_j$ is involved in self-occlusion relative to the view $I_k$. 

To evaluate $SC (p_j, I_k)$ for all the points $p_j$ of $C$ with respect to all input images $I_k$, we perform the following searching procedure for all the 2D pixel curves of all the input images. For any point $q$ on the image curve $C'_k$ in the view $I_k$, let  $N(q, d)$ denote the set of $q$'s neighboring pixels on $C_k$ whose distances to $q$ are at most $d$.  
% define $N(q; d) = \{u \| |u - q| \leq d, u\in C'_k u \}$,
We next find all the points on the 3D curve $C$ that are projected into the set $N(q; d)$, and denote these points by $\tilde N(q) \subset C$. Then we compute the standard deviation $\sigma$ of the distances of the points in $\tilde N(q)$ to their geometric centroid. The rationale of measuring $\sigma$ is that, there is self-occlusion observed at the pixel $q$, the points of  $\tilde N(q)$ should come from the same curve branches of $C$ so should be apart from each other, thus giving rise to a large standard deviation $\sigma$. Hence,  we set $SC (pi, I_k) :=TRUE$ for all the points $p_j$ in $\tilde N(q)$ if $\sigma \geq \sigma_0$ for a pre-specified threshold $\sigma_0$, because a large $\sigma$ means the likelihood that self-occlusion occurs at the point $q$. Otherwise, if $\sigma < \sigma_0$,  we set $SC (p_j, I_k) :=FALSE$ for all the points $p_j$ in $\tilde N(q)$. In this way, the label functions $SC (p_j, I_k)$ associated with all the points $p_i \in C$ are evaluated after checking all the images curve pixels in all the input images.

The information about self-occlusion allows us to ensure that only reliable image observation not involving self-occlusion is used for constructing the 3D skeletal curve network and estimating the radius of the thin structure. When a point $p_j \in C$ needs to be updated by minimizing the objective function $\tilde F$ in Eqn. (\ref{FD}), its associated error term $e_{k,j}$ (Eqn. (\ref{de})) is included $\tilde F$ only if $SC(p_j, I_k) = FALSE$, that is , if the point $p_j$ is not involved in self-occlusion with respect to the input view $I_k$. Similarly, when estimating the radius of the thin structure at $p_j$, the observation from the image $I_k$ should be used only if $SC(p_j, I_k) = FALSE$. The detailed computation of the radius function will be discussed shortly. 

\subsection{Initialization for optimization}
\label{sec:initialize}

We now discuss how to initialize the camera poses and the 3D curve network in order to proceed with iterative optimization described in Section \label{sec:iteration}. We first select thr first two frames (or two initial nearly input image frames), denoted as $I_1$ and $I_2$.  Since the two selected views are close to each other, their corresponding curve segments are close to each other, we compute a pixel correspondence between the curve segments using the curve matching method in~\cite{x}  (see~\figref{overview}~(b), \secref{initialStruct}). Then we jointly estimating a camera pose and a 3D point cloud using \red{bundle adjustment}. The connectivity of 3D points is constructed using a variant of spanning tree algorithm that allows the existence of cycles (\secref{spaningTree}). Note that the initial curve structure may easily be affected by self-occlusion of the 3D curve networks in the input views, which we will resolve by presenting a novel algorithm for detecting self-occlusion.
\james{We use the first two frames in the current implementation, but can the system still work from arbitrary two frames? Shall we conduct an experiment on different initial condition?}

% The system starts with reconstructing an initial 3D thin structure from 2D skeleton curves observed in two consecutive frames among the input image sequence (see~\figref{overview}~(b), \secref{initialStruct}).
% %
%
% This is done by computing a pixel correspondence between two 2D skeleton curves via a curve matching method~\cite{x} and then jointly estimating a camera pose and a 3D point cloud using \red{bundle adjustment}.
%
% The connectivity of 3D points is constructed using a variant of spanning tree algorithm that allows the existence of cycles (\secref{spaningTree}). 
%We build the connectivity of 3D points using a variant of spanning tree algorithm that accounts for the unique features of thin structure (\ie straightness and  cycles) (\secref{spaningTree}). 
%
% Note that the initial structure may easily suffer from noisy points and disconnected parts due to the inconsistency and occlusion occurred between two image observations.
%



\subsection{Surface reconstruction}
\label{sec:surf_reconstruct}
\subsubsection{3D radius estimation}
To generate the sweep surface, the radius of each skeleton curve point needs to be calculated. For each 3D curve point $p_j$ in $C_i$, we first find the 2D radius $\widetilde{r}_j^k$ of its correspondence $q_j^k$ of image $I_k$ by calculating the shortest distance from $q_j^k$ to the segmentation boundary. Then the 3D radius indicated from a single view
\begin{equation}
\overline{r}_j^k = \frac{\widetilde{r}_j^kdepth(p_j, k)}{f}
\end{equation}Where $f$ is the focal length of the camera.

\par
In ideal situations, to obtain the 3D radius of point $p_j$, we can fuse the the radius information from all the camera views by simply averaging them. However, due to the occlusion (WangPeng: figure is needed here.), the 2D radius estimation from some camera views could be inaccurate. Thus, we restrain the occlusion by the strategy introduced in \ref{sec:occlusion} and only consider the radius information of image $I_k$ with $SC(P_j, I_k) = FALSE$.

%

\subsubsection{Topology refinement}
A simple topological graph is not accurate enough for the final structure. Due to the ambiguity of junctions (Figure is needed here). To 

% old texts by Peng.

% %\begin{comment}
% \section{Peng's original texts}
% \section{Initialization}
% % \subsection{Pre-process}
% % Given segmented image $I^k$, we first apply thinning method to get new image $I^{k*}$ with one-pixel width curves. After thinning, for every pixel $p_i$ of $I^{k*}$ with value 1, we estimate its corresponding tangent vector through local weighted PCA: $$M_i^k \in \mathbb{R}^{2\times 2} = \sum_{x,y}{we^{-(x^2 + y^2)}I^{k*}_{p_i}[x,y]^\top[x,y]}$$ is computed and we get eigenvalues $\{\lambda^0, \lambda^2\}$ and eigenvectors $\{v^0, v^1\}$. $v^1$ is regarded as the tangent estimation of pixel $p_i$, and $s_i = \frac{\lambda^2}{\lambda^1 + \lambda^2}$ is the confidence of the tangent vector, indicating how "straight" this region is.

\subsection{Compute initial candidates}
In this step, we select two images $I^a, I^b$, and estimate initial poses and 3D points by optimizing a BA-like cost function.
\par
First, rough matching pairs $\{(p_i^a, v_i^a)\rightarrow (p_j^b, v_j^b)\}$ between these two images are calculated by using the combination of optical flow and shortest distance searching (Why optical flow here? Can we replace it with a curve matching algorithm?). 
\par
Assume $\pi(p_i^a, d_i^a, R^a, T^a)$ is the 2D point projected to the second image $I^b$ from the first image $I^a$, given depth $d_i^a$, rotation $R^a$ and translation $T^a$. Take $\{d_i^a\}, R^a, T^a$ as variables, for all matching pairs, a cost function is minimized:
$$\sum_{i,j} |bias_{i,j}\times v_j^b|^2 + w|bias_{i,j}\cdot v_j^b|^2 + \alpha\sum_i|d_i^a - 1|^2$$
Where $bias_{i,j} = \pi(p_i^a, d_i^a, R^a, T^a) - p_j^b$, and the second term is form regularization. $w$ and $\alpha$ are parameters and in our implementation $w = 0.5, \alpha = 0.01$.
\par
Through different initial value settings and minimizing this cost function, we will get several (usually 2-4 in our experiments) candidates of $(\{d_i^a\}, R^a, T^a)$ for the later iteration procedure.


At any time in the iteration procedure, the following information should be maintained: 
\begin{enumerate}
\item The global model $\{V, E\}$, including 3D point cloud $V = \{P_i \in \mathbb{R}^{3\times 1}\}$ and their linking information $E = \{(P_{a_i}, P_{b_i})\}$.
\item Information of active views. For every active views  $i$, we hold segmented and thinned maps $(I^i, I^{*i})$ and information of 2D local curve points $\{(p_k^i, v_k^i, s_k^i, r_k^i)\}$. 
\end{enumerate}
\par
Recall the principle mentioned before, we should keep the consistency between the global model and the observation of active views, while adding new image views could break this consistency. Thus we need to continuously update the model and active views, as the figure shows.
\begin{figure}[htp]
    \centering
    \includegraphics[width=7cm]{figure/iteration.png}
    \caption{}
    \label{fig:iteration}
\end{figure}
%

\textbf{Update linking edges}
\par
After the 3D model points have been updated, we need to recompute the topology of current model. We apply an algorithm (which is a bit like Kruskal algorithm), described as following:
\begin{enumerate}
\item First, we select edge candidates $E' = \{(P_{a_i}, P_{b_i} | \ |P_{a_i} - P_{b_i}| < \theta)\}$, where $\theta$ is a preset threshold.
\item At the same time we maintain a graph $G = (V, E)$, where $V = \{P\}$ and $E = \{\}$ (empty set) at the beginning.
\item Consider adding edges from $E'$ to $E$ by ascending order of the edge length. For each edge $(P_{a_i}, P_{b_i})$, if there isn't a path in $G$ from $P_{a_i}$ to $P_{b_i}$, or there is such a path but the length of the path is greater than some threshold, we add $(P_{a_i}, P_{b_i})$ to $E$.
\item Repeat 3 until all edges in $E'$ have been considered.
\end{enumerate}
\par
\textbf{Find matching from model points to active views}
\par
To implement 3D points updating process, we need to find their matching to active views first.
\par
A naive way to find curve matching between 2D and 3D is to project the 3D points to the active view and conduct 2D matching algorithm (For example, optical flow). But such kind of method can't solve the ambiguity problem due to 3D-2D overlapping. As the figure shows, the yellow point on the left is one 2D point of the model's projection to the active view, and the right is the observation of current active view. If we only consider 2D to 2D matching, we then don't know if it should match the red point or the green point.
\begin{figure}[htp]
    \centering
    \includegraphics[width=6cm]{figure/matching.png}
    \caption{}
    \label{fig:matching}
\end{figure}
\par
Thus we conduct an 3D-2D matching algorithm, considering the context in the current iterating 3D model. For the matching from model points to a single view, the matching method can be described as following:
\par
\begin{enumerate}
\item For each model point $P_i$, we project it to the current view and plus it with optical flow, say $q_i = \pi(RP_i + T) + flow(\pi(RP_i + T))$.
\item 
\end{enumerate}
\par
\textbf{Adding new points}
\par
Currently: voxel voting (TODO, change to a better method)
\section{Refinement}
\par
TODO
\par
%\end{comment}

==> figure/fig_compare_sfm.tex <==
\def\sfmCaseA{modelA}
\def\sfmCaseB{modelA}
\def\sfmCaseC{modelA}
\def\sfmCaseD{modelA}

\newcommand{\SfMEntry}[2]{figure/models/#1/#1_#2}
\def\SfMDivider{0.18}

\begin{figure*}[!t]
    % ===== Row 1 ===== 
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseA}{RGB}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseA}{PMVS}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseA}{COLMAP}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseA}{RGB}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseA}{Final}}}
    \\
    \vspace{1mm}
    % ===== Row 2 ===== 
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseB}{RGB}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseB}{PMVS}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseB}{COLMAP}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseB}{RGB}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseB}{Final}}}
    \\
    \vspace{1mm}
    % ===== Row 3 ===== 
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseC}{RGB}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseC}{PMVS}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseC}{COLMAP}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseC}{RGB}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseC}{Final}}}
    \\
    \vspace{1mm}
    % ===== Row 4 ===== 
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseD}{RGB}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseD}{PMVS}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseD}{COLMAP}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseD}{RGB}}}
    \hfill
    \mpage{\SfMDivider}{\includegraphics[width=\linewidth]{\SfMEntry{\sfmCaseD}{Final}}}
    \\
    % ===== Button line labels =====
    \mpage{\SfMDivider}{Input image \\ (PMVS & COLMAP)}
    \mpage{\SfMDivider}{PMVS}
    \mpage{\SfMDivider}{COLMAP}
    \mpage{\SfMDivider}{Input image (Ours)}
    \mpage{\SfMDivider}{Ours}
    
    
    \caption{
    \hl{
    \tb{Comparisons with structure-from-motion methods.} 
    \james{} 
    }
    }
    \label{fig:compare_sfm}
\end{figure*}

==> figure/fig_formulation.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7 \linewidth]{figure/formulation}
    \caption{
    \hl{
    \tb{}
    }
    }
    \label{fig:formulation}
\end{figure}


==> figure/fig_limitations.tex <==
\begin{figure}[!h]
    \mpage{0.374}{\includegraphics[width=\linewidth]{figure/fig_limitations_1}}
    %\hfill
    \mpage{0.576}{\includegraphics[width=\linewidth]{figure/fig_limitations_2}}
    %
    
    \caption{\hl{Our algorithm can not handle objects with extremely dense curves, such as steel wire ball.}}
    \label{fig:limitations}
\end{figure}


==> figure/fig_segmentation.tex <==
\begin{figure}[htb]
    %\hfill
    %\mpage{0.31}{\includegraphics[width=\linewidth]{figure/segmentation_noise_real_a}}
    %\mpage{0.31}{\includegraphics[width=\linewidth]{figure/segmentation_noise_real_b}}
    %\mpage{0.31}{\includegraphics[width=\linewidth]{figure/segmentation_noise_real_c}}
    %\\
    % ===== Button line labels =====
    % \mpage{0.45}{(a)}
    % \mpage{0.45}{(b)}
    
  \mpage{0.23}{\includegraphics[width=\linewidth]{figure/segmentation_noise_synthetic_clear}}
    \mpage{0.23}{\includegraphics[width=\linewidth]{figure/segmentation_noise_synthetic_shaking}}
    \mpage{0.23}{\includegraphics[width=\linewidth]{figure/segmentation_noise_synthetic_polluting}}
    \mpage{0.23}{\includegraphics[width=\linewidth]{figure/segmentation_noise_synthetic_missing}}
 \\
 \mpage{0.23}{clear}
 \mpage{0.23}{shaking}
 \mpage{0.23}{polluting}
 \mpage{0.23}{missing}
    
    \caption{\hl{Different types of segmentation noise.}}
    \label{fig:segmentation}
\end{figure}


==> figure/tbl_evaluate_comparison.tex <==
\begin{table}[!b]\tiny
    \centering
    \caption{\james{let's remove this table and discuss the performance via text...}}
    \resizebox{0.8\linewidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            PMVS &  COLMAP & Li et al. [2018] & Ours \\
            \midrule
            % Blender && 0.0078 & 2.4848 \\
            % 2.0585 & 1.4200 & 0.8900 & 0.4073 \\
            0.00338 & 0.00233 & 0.00146 & 0.00067 \\
            \bottomrule
        \end{tabular}
    }
    \label{tbl:evaluate_comparision}
\end{table}

==> figure/tbl_evaluate_synthetic_shake.tex <==
\begin{table}[t]\tiny
    \centering
    \caption{Quantitative evaluation on the sensitivity to different degrees of camera shake. Please refer to~\secref{metric_compare} for the definition of error metrics.}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{ccccccc}
            \toprule
            && RE & RRE & PE & TPE & TRE \\
            \midrule
            % Blender && 0.0027 & 0.0030 & 0.0032 \\
            Cam. shake (small) && 0.000651 & 0.0807 & 0.0014 & 48/48 & 48/50 \\
            Cam. shake (medium) && 0.001144 & 0.1418 & 0.0024 & 44/47 & 44/50\\
            Cam. shake (large) && 0.003349 & 0.4163 & 0.0043 & 41/47 & 41/50\\
            % \hline\hline
            % Boundary Noise (0.1) && 0.000727 & 0.0900 \\
            % Boundary Noise (0.3) && 0.000765 & 0.0947 \\
            % Boundary Noise (0.5) && 0.000891 & 0.1102 \\
            \bottomrule 
        \end{tabular}
    }
    \label{tbl:evaluate_synthetic_shake} 
\end{table}
\begin{comment}
\end{comment}

==> setup/graphicspath.tex <==
\graphicspath{{figure}, {images}, {example}}
%\DeclareGraphicsExtensions{.pdf,.jpeg,jpg,.png}


==> setup/symbols_backup.tex <==
% Define math symbols that appear in the texts

% Input RGB images
\def\imgSymbol{I}
\def\inputI{\mathbf{\imgSymbol}}            % Set
\newcommand{\inputIk}[1]{\imgSymbol_{#1}}   % Element

% Segmented images
\def\segSymbol{M}
\def\segI{\mathbf{\segSymbol}}                  % Set
\newcommand{\segIk}[1]{\segSymbol_{#1}}         % Element

% Thinning images
\def\thinSymbol{\bar{I}}
\def\thinI{\mathbf{\thinSymbol}}                % Set
\newcommand{\thinIk}[1]{\thinSymbol_{#1}}       % Element

% Camera poses
\def\rotSymbol{R}
\newcommand{\camRk}[1]{\rotSymbol_{#1}}          % Camera rotation component

\def\tranSymbol{T}
\newcommand{\camTk}[1]{\tranSymbol_{#1}}        % Camera translation component

% 2D skeletal curves
\def\skelSymbol{\tilde{C}}
\def\skelC{\mathbf{\skelSymbol}}                % Set
\newcommand{\skelCk}[1]{\skelSymbol_{#1}}       % Element

\def\frameNum{K}                                % Number of frames
\def\curvePntNum{m}                             % Number of 3D points
\def\skelPntNum{n}                              % Number of 2D points

% 3D curve structure
\def\curveSymbol{C}
\def\curveStruct{\curveSymbol}
\newcommand{\curveProjk}[1]{\curveSymbol'_{#1}}

\def\occluFunc{\mathbb{I}_{occ}}

% Error metrics
\def\RE{RE} % Reconstruction Error
\def\RRE{RRE} % Relative Reconstruction Error
\def\RPE{RPE} % Relative Pose Error
\def\PE{PE} % Projection Error
\def\TPE{TPE} % Topology Error: Precision
\def\TRE{TRE} % Topology Error: Recall

%\def\RE{Rec. Err.} % Reconstruction Error
%\def\RRE{Rel. Err.} % Relative Reconstruction Error
%\def\RPE{RPE} % Relative Pose Error
%\def\PE{Proj. Err.} % Projection Error
%\def\TPE{Topo. Pre.} % Topology Error: Precision
%\def\TRE{Topo. Rec.} % Topology Error: Recall


